Feature Modulation to Improve Struggle Detection in Web Search: A Psychological Approach

Searcher struggle is important feedback to Web search engines. Existing Web search struggle detection methods rely on effort-based features to identify the struggling moments. Their underlying assumption is that the more effort a user spends, the more struggling the user may be. However, recent studies have suggested this simple association might be incorrect. This paper proposes a new feature modulation method for struggle detection and refers to the reversal theory in psychology. The reversal theory (RT) points out that instead of having a static personality trait, people constantly switch between opposite psychological states, complicating the relationship between the efforts they spend and the level of frustration they feel. Supported by the theory, our method modulates the effort-based features based on RT's bi-modal arousal model. Evaluations on week-long Web search logs confirm that the proposed method can statistically significantly improve state-of-the-art struggle detection methods.

==> Random.tex <==

The two random variables follow two different normal distributions with different means and variances, respectively: %Here we model the feature value distribution as $P(X_i|\textrm{means-ends})$. The arousal (effort) distribution in telic state is %$X_{telic}

=====

%Situational triggers are interesting because they are something we can control to some extent. To reverse from telic to paratelic state, situational triggers can be removal of threat, entertainment, or humor. To reverse from paratelic to telic, situational triggers can be unavoidable tasks, sudden threat, and need for strategic decisions~\cite{personalitydynamics}.  


% Our work sees search struggles as a type of
% psychological experience, which starts from subjective feelings and reaches out to behavior, physiology, and performance. As for the extent of observable behavioral effort during search, it alone doesn't characterize search as struggling or not, unless considered under the motivation dynamics. %After categorizing user motivation using RT, we point out that users are more tolerant towards struggles when they are searching for non-goal-oriented tasks than for goal-oriented tasks. 
% In this paper, we only use search task type  as the main contingent factor, which corresponds to the ``means-end" motivational dimension, to induce reversals and to detect struggles. However, struggle itself can be a trigger for motivational state reversal. It would be interesting to study how earlier struggles would impact motivational states and later detection. 

=====
%Based on what's suggested by RT and confirmed by our tests, 



%=======


This diminishes the distinguishing power of effort-based features when using them in classifiers. 

=====

%Gradient Boosted Decision Trees (GBDT) 

\grace{Jiyun, this para is temporarily put here. I tend to delete them. But please answer my questions.}
Features used in this process include similarity features between the URL and each taxonomy name \grace{Jiyun, you only used the name of a taxonomy? I know the url text (not the document it links to but the link text) is used from the url side. What do you use from the taxonomy side?} , such as embedding similarity \grace{what is embedding similarity???} and tf-idf. \jiyun{Your guess in the next paragraph is right. At Pinterest, we map each web document to a taxonomy name by a ML approach. The features  include: 1) embedding similarity. This is done by: a) represent the web document as  embeddings, b) represent the taxonomy as embeddings (word2vec is one of them. We have text based embedding for document and taxonomy entities, we also have graph based embeddings for web and taxonomy entities) and calculate  similarity scores, 2) tf-idf scores. (you can think the web document as the ``query'', we have candidate taxonomy entities, they are the retrieval ``documents'' in a way) and some other features (e.g. popularity feature, what's the most popular taxonomy label, user gives this document). I'm a bit ambiguous here, bc it is done by another team. I just used their results. At Pinterest, a taxonomy name/entity also has a bag of words and other information to support its definition.} 

=======

$M$ is a threshold selected by grid search. In our experiment, M=15, it is when the two states' average $ExploreScore$ are statistically significantly different at significant level $\alpha=.05$. \grace{Jiyun, chicken and egg problem?} \grace{why a grid search needs a significant level? Why $\alpha$ is needed here and why it is 0.05?} \jiyun{We want the groups to be as different as possible but also have relatively enough amount of sessions in each group. 15\% is a good cut off for our dataset.} 


A session's task type is determined by the search results' content in the session. 

=======

Other topic categories, such as ``Travel", are ignored because it is difficult to judge whether some of these sampled sessions are telic or paratelic sessions. As a result, we conclude that they are not representative enough in our dataset. In the end, every session in our analysis has been put into a telic or paratelic state.

=====

%%% the following paragraphs may be useful
%First, we try to properly pick some of these variables and map them into the latent binary, forming different coarse mappings. Second, according to the mappings we group some of the sessions, each into one of the two systems, and  adjust the sessions' feature magnitudes using a Bayesian scaling method to move the two curves together. Third, the modulated features were fed into a binary classifier to perform struggle detection. 

%\begin{figure}[t]
% \includegraphics[width=0.9\linewidth, height=4.8cm]{pics/effort_bias_task_based}
%   \caption{Effort bias based on task types. }
%   \label{fig-task-bias} 
%\end{figure}
%
%\begin{figure}[t]
% \includegraphics[width=0.9\linewidth, height=4.8cm]{pics/effort_bias_user_based}
%   \caption{Effort bias based on user types. }
%   \label{fig-user-bias} 
%\end{figure}

===========

%The feature values were all normalized into $[0,1]$ before being counted into the average. For example, for effort spent on querying, we first normalized the feature values in the ``efforts to query'' group into the same range of [0,1] and then took the average of the  normalized values. This group of features includes the numbers of queries and unique queries, the avg. numbers of terms and characters, and the ratio of manually typed queries. 
%This was performed twice, one for sessions in the negativistic state and the other for sessions in the conformist state. 

=======
%When $\alpha=.05$, M=15. 

=======
 
depicts RT's arousal model with both ``means-ends" and ``rules" interplaying. 
====

RT's modal of arousal also studies their joint impact on happiness and efforts. 

======

%The first two RT dimensions, ``means-ends" and ``rules", are related to completing tasks and exploring possibilities. They are relevant to Web search and hence targets of our study. The last two, ``transactions" and ``relationships", describe interpersonal interactions and are not directly relevant to this work. 


======
Struggles often appear in complex search tasks where the information need 


are built up over time and often show up in multi-query search sessions. A {\it session} is a sequence of querying-and-retrieval activities centering around a search task; it is the target under study in this work. 

======

\begin{comment}
We ran struggle detection classification experiments twice, once  before using feature modulation and another time after it.  

{\noindent} {\bf Before:}  In Tables \ref{tab-result-1} and \ref{tab-result-pc-2},  runs without ``FM'' suffix report the struggle detection results for the Mobile and the PC search logs, respectively, without feature modulation (FM). 

The Transformer model performs better than the other predictive models. It achieves 0.8811 accuracy in mobile search (Table \ref{tab-result-1}) and 0.8813 accuracy in search using PCs (Table \ref{tab-result-pc-2}), which is a statistically significant improvement over the state-of-the-art baseline Hassan et al. \cite{Hassan:2014:SED:2556195.2556221}. It suggests that the features we used are highly effective in predicting user struggles, even before we use feature modulation.
\end{comment}


====== 
%% motivate what to do from the theory 
%Note the modulation is done over the features. This is because our features are basically indicators of different kinds of efforts. In the model of arousal, they correspond to the x-axis, the arousal level. Based on the same mode of arousal, what struggle detection transformed into is the right lower corner of happiness level (the y-axis). Alternatively, the modeling can be achieved by a mixture of two Gaussian models with the use of a generative classifier. However, in this paper, we take a discriminating  approach and focus on how to reduce the bias between the two curves. 
==

%Figure \ref{fig-annotation-example} shows the query logs for (a) a struggling session on ``hair styles for dark skins" and (b) a non-struggling session on ``proposing ideas". 



% \begin{figure}[t]
%  \includegraphics[width=0.9\linewidth]{pics/fig-annotation-examples} 
%  \caption{Struggling vs. non-struggling sessions. } 
%      \label{fig-annotation-example} 
% \end{figure}


%This is an important distinction to make because a user can be struggling, but still be satisfied in the end. For example, if a user is trying to find the answer to a certain question and has to try many different queries because they cannot find what they're looking for, they may get frustrated even if they do end up finding what they're looking for \cite{Hassan:2014:SED:2556195.2556221}. While some other studies focus on determining if a user is {\it satisfied} with the results of a search, this research is specifically focused on determining if a user is {\it struggling} during the search process.


 
 %Fig. \ref{fig-annotation-example} (b) is an example of a struggling session. On March 11, 2015, the searcher tried to find information about how to delete Myspace accounts, however, struggles happened in the process of locating a useful webpage. Although there were several web pages talking about how to delete the account, they were from an outdated Myspace version and thus were non-relevant. The user comprised and changed queries to search for how to delete photos. Eventually it became a successful session since the user was able to locate a relevant URL in the end. However, it took her a lot of effort to finish the session, which constitutes a struggling session. 


%For example, in the first search session of Fig. \ref{fig-annotation-example} (a), the searcher found Fresenius' stock price by one query and one click. Also in the second search session (Fig. \ref{fig-annotation-example} (a)), the user was smoothly exploring animation clips about the gummy bear. 
%The second session in Fig. \ref{fig-annotation-example} is a non-struggling session that consumed a good amount of user effort. However, the user did not mind to spend  time on many gummy bear videos as long as they were fun. It was indeed a non-goal-oriented  search task. 


====

%% identify ODP from url links
%First, we extract the ODP category for each search session from clicked URLs. To do that, we tokenize the clicked URL and match its tokens one by one from the right most with ODP labels until a match is found. Once a match is identified, we label the URL with the top two levels in the ODP hierarchy. The exceptions are for the ``Regional'' and ``World'' categories -- we use their most specific categories rather than the top two levels. This is because the top two levels for those categories are too general to be informative. Then, we select the most frequent label of all the ODP labels assigned to the clicked URLs in the session as the topic label of the session. 


==================



\begin{comment}
%\textbf{ZeroRule} is a common baseline in the machine learning community which classifies all instances using the majority label in the ground truth.
%\textbf{MART\_SUB} uses all features reported in \cite{Hassan:2014:SED:2556195.2556221} and is trained using MART. \textbf{SVM} trains an SVM model using all features in Table \ref{tab-features}. 
%\textbf{LM} trains a logistic regression model using all features. \textbf{MART} trains a MART model using all features. And \textbf{NeuralNetwork} trains a three-layer neural network model using all features. All above runs are conducted for mobile search. Here \textbf{SVM} and \textbf{LM} are linear models, while \textbf{MART\_SUB}, \textbf{MART} and \textbf{NeuralNetwork} are non-linear models.

%We report Accuracy, Precision and Recall for the positive class (``Struggle'') and Precision and Recall for the negative class (``non-struggling''). Among all models, MART achieve 2.88\% improvement of accuracy over baseline MART\_SUB.  This improvement is statistically significant. It also achieves the highest Positive Precision score. It suggests that our features are highly effective in predicting user struggles in mobile search.

%It is worth pointing out that high Positive Precision is valuable in optimizing search engine performance. Research \cite{Savenkov:2014:HEE:2600428.2609523} suggests that providing precise and specific assistance can improve search success and user experience however generic or misleading assistance increases user struggles. Hence precisely predicting user struggles is more important than predicting ``non-struggling'' tasks. It helps move towards providing desired assistance to users. In this sense, SVM is our best linear model, and  MART is our best non-linear model.

%We also train SVM, LM, MART\_SUB, MART and NeuralNetwork models on the 365 tasks labeled for detecting struggles in search using PCs and report the results in Table \ref{tab-result-pc-2}. 

\end{comment}
 %majority vote, logistic regression\cite{friedman2000additive}, SVM\cite{Cortes:1995:SN:218919.218929}, MART\cite{friedman2001greedy} and Transformer \cite{10.5555/3295222.3295349}. All classifiers are trained and validated with a 10-fold cross-validation. 
